Multimessenger observations of counterparts to IceCube-190331A

High-energy neutrinos are a promising tool for identifying astrophysical sources of high and ultra-high energy cosmic rays (UHECR). Prospects of detecting neutrinos at high energies ($\gtrsim$TeV) from blazars have been boosted after the recent association of IceCube-170922A and TXS 0506+056. We investigate the high-energy neutrino, IceCube-190331A, a high-energy starting event (HESE) with a high likelihood of being astrophysical in origin. We initiated a Swift/XRT and UVOT tiling mosaic of the neutrino localisation, and followed up with ATCA radio observations, compiling a multiwavelength SED for the most likely source of origin. NuSTAR observations of the neutrino location and a nearby X-ray source were also performed. We find two promising counterpart in the 90% confidence localisation region and identify the brightest as the most likely counterpart. However, no Fermi/LAT $\gamma$-ray source and no prompt Swift/BAT source is consistent with the neutrino event. At this point it is unclear whether any of the counterparts produced IceCube-190331A. We note that the Helix Nebula is also consistent with the position of the neutrino event, and we calculate that associated particle acceleration processes cannot produce the required energies to generate a high-energy HESE neutrino.

==> changes.tex <==
% Changes to aastex61 default settings:
% Reduced ``affiliation'' fontsize
\makeatletter
\def\frontmatter@affiliationfont{\normalfont\scriptsize\it
\ifmodern\baselineskip=6pt\fi
\iflongauthor\else
\rightskip-12pt plus 1fil
\leftskip6pt \parindent-4pt
\fi
}%

% Less space between authors & affiliations
\def\@affil@script#1#2#3#4{%
%\ifmodern
\iffirstaffil\vskip6pt 
\global\firstaffilfalse\fi%\fi
 \@ifnum{#1=\z@}{}{%
  \par
  \begingroup
   \frontmatter@affiliationfont
   \@ifnum{\c@affil<\affil@cutoff}{}{%
\def\one{#1}
\ifnum\one<\largestAffilNum
%% this makes the numbers
   \def\@thefnmark{#1}\@makefnmark\fi
\ifnum\one=\largestAffilNum
   \def\@thefnmark{#1}\@makefnmark\fi
   }%
% this makes the text
\ifnum\one<\largestAffilNum
   \ignorespaces#3%
\fi
\ifnum\one=\largestAffilNum
   \ignorespaces#3%
\fi
   \@if@empty{#4}{}{\frontmatter@footnote{#4}}%
   \par
  \endgroup
 }%
}%
\makeatother
